Non-commutative Frobenius characteristic of generalized parking functions -- Application to enumeration

We give a recursive definition of generalized parking function that allows us to view them as a species. From there we compute a non-commutative characteristic of the generalized parking function module, and deduce some enumeration formulas of structures and isomorphism types. We give as well an interpretation in several bases of non-commutative symmetric functions. Finally, we investigate an inclusion-exclusion formula given by Kung and Yan.

==> schema_construction.tex <==
\vcenter{\hbox{\begin{tikzpicture}
    \draw[thick, rounded corners] (0,0) rectangle (4,2);
    \fill[red] (2,.5) circle (.5ex);
    \foreach \x in {15,30,...,160} {
        \draw (2,.5) ++(\x:.5ex) --++(\x+10:1)[fill] circle (.3ex);
    }
    \draw[red] (2.5,.5) arc (25:155:.55);
    \node at (1, .3) {$\pfc{\speciesA}$};
    \end{tikzpicture}}}
    \quad = \quad
    \vcenter{\hbox{\begin{tikzpicture}[scale=.3]
   \def\x{20}
   \def\y{20}
    \foreach \i in {0,...,\x} { \draw [very thin,gray] (\i,0) -- (\i,\y); }
    \draw [very thin,gray] (0,0) -- (\x,0);
    \foreach \i in {2,4,...,\y} {
        \draw [very thin,gray] (0,\i) -- (\x,\i);
    }
    \node[red] at (3, 14) {$\seqPF$};
    \draw[thick, red] (0,0) -- (0, 4) -- (2,4) -- (2,6) -- (3,6) -- (3,10) 
                            -- (4, 10) -- (4, 16) -- (10, 16) -- (10, 18) 
                            -- (16, 18) -- (16, 20) -- (20, 20);
    % \node[red] at (9, 12) {$\species^{\blacktriangle^\an}$};
    \draw[thick, blue!60] (0, 2) -- (2.1,2) -- (2.1,5.9) -- (6, 6) -- (6, 10) 
                                 -- (12, 10) -- (12,17.9) -- (20, 17.9);
    \node (q0) at (1,.5) [scale=.9,token=1,red] {};
    \node (0) at (.5,1.5) [scale=.6,token=1] {};
    \node (1) at (1.5,1.5) [scale=.6,token=1] {};
    \path (q0) edge (0) edge (1);
    %
    \node (q1) at (2.5,3) [scale=.9,token=1,red] {};
    \node (q2) at (4,4.5) [scale=.9,token=1,red] {};
    \foreach \i in {2,...,5}
        \node (\i) at (\i.5,5.5) [scale=.6,token=1] {};
    \path (q2) edge (2) edge (3) edge (4) edge (5);
    \node (q3) at (6.5,7) [scale=.9,token=1,red] {};
    \node (q4) at (9,8.5) [scale=.9,token=1,red] {};
    \foreach \i in {6,...,11}{
        \node (\i) at (\i.5,9.5) [scale=.6,token=1] {};
        \path (q4) edge (\i);
    };
    \foreach \i in {11,13,15}
        \node (q\i) at (12.5,\i) [scale=.9,token=1,red] {};
    \node (q5) at (16,16.5) [scale=.9,token=1,red] {};
    \foreach \i in {12,...,19}{
        \node (\i) at (\i.5,17.5) [scale=.6,token=1] {};
        \path (q5) edge (\i);
    };
    \node at (2.5, 1) {$\speciesA$};
    \node at (3.5, 3) {$\speciesA$};
    \node at (6, 5) {$\speciesA$};
    \node at (7.5, 7) {$\speciesA$};
    \node at (10.5, 8.5) {$\speciesA$};
    \node at (13.5, 11) {$\speciesA$};
    \node at (13.5, 13) {$\speciesA$};
    \node at (13.5, 15) {$\speciesA$};
    \node at (20.5, 17) {$\speciesA$};
    \node (qE) at (10.5,2) [scale=.9,token=1,red] {};
    \node at (11.5,.5) {$(\speciesA^{\seqPFn{1}})_2$};
    \foreach \i in {0,1} 
        \path[gray,thick] (qE) edge (q\i);
    \node (qA) at (12.5,4) [scale=.9,token=1,red] {};
    \node at (11.5,4.8) {$(\speciesA^{\seqPFn{3} - \seqPFn{1}})_4$};
    \path[gray,thick] (qA) edge (q2);
    \node (qF) at (14.5,6) [scale=.9,token=1,red] {};
    \node at (18.5,6.5) {$(\speciesA^{\seqPFn{7} - \seqPFn{3}})_6$};
    \foreach \i in {3,4} 
        \path[gray,thick] (qF) edge (q\i);
    \foreach \i in {11,13,15} 
        \path[gray,thick] (qF) edge (q\i);
    \node (qbl) at (16.5,3) [scale=.9,token=1,red] {};
    \node (qG) at (16,14) [scale=.9,token=1,red] {};
    \node at (19.9,14) {$(\speciesA^{\seqPFn{13} - \seqPFn{7}})_8$};
    \path[gray,thick] (qG) edge (q5);
    \path[thick] (qbl) edge (qE) edge (qF) edge (qA) edge (qG);
    \node at (18.5,3) {$\pfc{\speciesA}$};
    \end{tikzpicture}}}
